Mathematical Language Models: A Survey

In recent years, there has been remarkable progress in leveraging Language Models (LMs), encompassing Pre-trained Language Models (PLMs) and Large-scale Language Models (LLMs), within the domain of mathematics. This paper conducts a comprehensive survey of mathematical LMs, systematically categorizing pivotal research endeavors from two distinct perspectives: tasks and methodologies. The landscape reveals a large number of proposed mathematical LLMs, which are further delineated into instruction learning, tool-based methods, fundamental CoT techniques, advanced CoT methodologies and multi-modal methods. To comprehend the benefits of mathematical LMs more thoroughly, we carry out an in-depth contrast of their characteristics and performance. In addition, our survey entails the compilation of over 60 mathematical datasets, including training datasets, benchmark datasets, and augmented datasets. Addressing the primary challenges and delineating future trajectories within the field of mathematical LMs, this survey is poised to facilitate and inspire future innovation among researchers invested in advancing this domain.

==> secs/Evaluation.tex <==
\section{Evaluation Metrics}
\label{Evaluation}
% SOCREVAL
To evaluate the arithmetic and math ability of language models, various math
word problems datasets \cite{saxton_analysing_2019,hendrycks2021measuring,cobbe_training_2021,kushman-etal-2014-learning} are designed with difference metrics \cite{wang2021gpt,chung2022scaling,thoppilan2022lamda,yuan2023well}. 
For example, \cite{nogueira2021investigating,wang2021exploring,muffo_evaluating_nodate} evaluate pretrained language models on simple
arithmetic expressions including addition, subtraction and multiplication.
Moreover, \cite{shakarian2023independent,frieder2023mathematical} evaluate ChatGPT's mathematical ability independently. 

In this paper, we organize the frequently used datasets and evaluation metrics for mathematical language models.

Word predictions in language modeling are typically evaluated with classification metrics such as
accuracy or perplexity. Numeric predictions, on the
other hand, are evaluated with regression metrics
such as mean absolute error, root mean squared error, or their log and percentage variants \cite{berg-kirkpatrick-spokoyny-2020-empirical}. \cite{spithourakis2018numeracy} also propose an Adjusted Perplexity
metric to cancel the effect of the out-of-vocabulary
rate on the perplexity of numeric tokens.

Math Dataset \cite{hendrycks2021measuring}, performs Extra Match(EM) of answers by forcing the final boxed answers to follow consistent formatting rules. The Microsoft team at AGIEval Dataset \cite{zhong2023agieval} employs Exact Match and F1 metrics for fill-in-the-blank questions, as well as evaluating the model using human assessment in terms of semantic understanding capability, knowledge utilization, and reasoning quality.

In order to assess the quality of model inference chains, a more intuitive approach is to compare these generated chains with human-constructed chains, known as reference-based inference assessment, and there are also reference-less assessment methods such as scoring via large language models \cite{he2023socreval}.
